First-order Conditions for Optimization in the Wasserstein Space

We study first-order optimality conditions for constrained optimization in the Wasserstein space, whereby one seeks to minimize a real-valued function over the space of probability measures endowed with the Wasserstein distance. Our analysis combines recent insights on the geometry and the differential structure of the Wasserstein space with more classical calculus of variations. We show that simple rationales such as "setting the derivative to zero" and "gradients are aligned at optimality" carry over to the Wasserstein space. We deploy our tools to study and solve optimization problems in the setting of distributionally robust optimization and statistical inference. The generality of our methodology allows us to naturally deal with functionals, such as mean-variance, Kullback-Leibler divergence, and Wasserstein distance, which are traditionally difficult to study in a unified framework.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> old/old.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%
% Proof alpha convexity OT discrepancy
%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
\item Let $\mu_0,\mu_1,\tilde\mu\in\Pp{2}{\reals^d}$, and let $\gamma\in\setOptimalPlans{\mu_0}{\mu_1}$. Recall that the generalized geodesic between between $\mu_0$ and $\mu_1$, with base $\tilde\mu$ is 
\begin{equation}\label{eq:optimal transport discrepancy alpha convexity geodesic}
    \mu_t=\pushforward{((1-t)\proj_2+t\proj_3)}\gamma,
\end{equation}
where $\gamma\in\Pp{2}{\reals^d\times\reals^d\times\reals^d}$ with $\pushforward{(\proj_{12})}\gamma\in\setOptimalPlans{\tilde\mu}{\mu_0}$ and $\pushforward{(\proj_{23})}\gamma\in\setOptimalPlans{\tilde\mu}{\mu_1}$. Note that
\begin{equation}\label{eq:optimal transport discrepancy alpha convexity marginals}
    \pushforward{(\proj_2)}\gamma = \mu_0,
    \qquad 
    \pushforward{(\proj_3)}\gamma = \mu_1.
\end{equation}
The proof simply consists of exploiting the convexity of $c(\cdot,y)$; i.e., 
\begin{equation}\label{eq:optimal transport discrepancy alpha convexity convexity c}
    -c((1-t)x_0+tx_1,y)
    \leq 
    -(1-t)c(x_0,y) - tc(x_1,y) -\frac{\alpha}{2}t(1-t)\norm{x_0-x_1}^2.
\end{equation}
To start, we need some notation: We denote by $\tilde\gamma$ plans in $\Pp{2}{\reals^d\times\reals^d}$ and by $\bar\gamma$ plans between a probability measure in $\reals^d\times\reals^d\times\reals^d$ and one $\reals^d$ (in particular, $\gamma$ and $\bar\mu$).
Moreover, \nlmargin{from}{complete}, for any $\nu_0\in\Pp{}{X}$ and any $\nu_1\in\Pp{}{Y}$
\begin{equation}\label{eq:optimal transport discrepancy alpha convexity property set plans}
    \pushforward{(f\times \Id)}\setPlans{\nu_0}{\nu_1}
    =
    \setPlans{\pushforward{f}\nu_0}{\nu_1}
\end{equation}    
Then, 
\begin{align*}
    -\cost(\mu_t)
    &=
    -\min_{\tilde\gamma\in\setPlans{\mu_t}{\bar\mu}}
    \int_{\reals^d\times\reals^d}c(x,y)\d\tilde\gamma(x,y)
    \\
    \overset{\eqref{eq:optimal transport discrepancy alpha convexity geodesic}}&{=}
    -\min_{\tilde\gamma\in\setPlans{\pushforward{(((1-t)\proj_2+t\proj_3)\times \Id)}\gamma}{\bar\mu}}
    \int_{\reals^d\times\reals^d}c(x,y)\d\tilde\gamma(x,y)
    \\
    \overset{\eqref{eq:optimal transport discrepancy alpha convexity property set plans}}&{=}
    -\min_{\tilde\gamma\in\pushforward{(((1-t)\proj_2+t\proj_3)\times \Id)}\setPlans{\gamma}{\bar\mu}}
    \int_{\reals^d\times\reals^d}c(x,y)\d\tilde\gamma(x,y)
    \\
    &=
    -\min_{\bar\gamma\in\setPlans{\gamma}{\bar\mu}}
    \int_{\reals^d\times \reals^d\times \reals^d\times \reals^d}
    c(x,y)\d\pushforward{(((1-t)\proj_2+t\proj_3)\times \Id)}\bar\gamma(\tilde x,x_0,x_1,y)
    \\
    &=
    -\min_{\bar\gamma\in\setPlans{\gamma}{\bar\mu}}
    \int_{\reals^d\times \reals^d\times \reals^d\times \reals^d}
    c((1-t)x_0+tx_1,y)\d\bar\gamma(\tilde x,x_0,x_1,y)
    \\
    &=
    \max_{\bar\gamma\in\setPlans{\gamma}{\bar\mu}}
    \int_{\reals^d\times\reals^d\times\reals^d\times\reals^d}
    -c((1-t)x_0+tx_1,y)\d\bar\gamma(\tilde x,x_0,x_1,y)
    \\
    \overset{\eqref{eq:optimal transport discrepancy alpha convexity convexity c}}&{\leq}
    \max_{\bar\gamma\in\setPlans{\gamma}{\bar\mu}}
    \int_{\reals^d\times\reals^d\times\reals^d\times\reals^d}
    -(1-t)c(x_0,y)-tc(x_1,y)-\frac{\alpha}{2}t(1-t)\norm{x_0-x_1}^2\d\bar\gamma(\tilde x,x_0,x_1,y)
    \\
    &= 
    \begin{aligned}[t]
    &\max_{\bar\gamma\in\setPlans{\gamma}{\bar\mu}}
    \int_{\reals^d\times\reals^d\times\reals^d\times\reals^d}
    -(1-t)c(x_0,y)-tc(x_1,y)\d\bar\gamma(\tilde x,x_0,x_1,y)
    \\
    &-\frac{\alpha}{2}t(1-t)\int_{\reals^d\times\reals^d\times\reals^d}\norm{x_0-x_1}^2\d\gamma(\tilde x,x_0,x_1).
    \end{aligned}
    \\
    &\leq 
    \begin{aligned}[t]
    &\max_{\bar\gamma\in\setPlans{\gamma}{\bar\mu}}
    \int_{\reals^d\times\reals^d}
    -(1-t)c(x_0,y)\d\pushforward{(\proj_{2}\times\Id)}\bar\gamma(x_0,y)
    \\
    &+
     \int_{\reals^d\times\reals^d}
    -t c(x_1,y)\d\pushforward{(\proj_{3}\times\Id)}\bar\gamma(x_1,y)
    -\frac{\alpha}{2}t(1-t)\wassersteinDistance{2}{\mu_0}{\mu_1}^2
    \end{aligned}
    \\
    &\leq 
    \begin{aligned}[t]
    &\max_{\bar\gamma_0\in\setPlans{\gamma}{\bar\mu}}
    \int_{\reals^d\times\reals^d}
    -(1-t)c(x_0,y)\d\pushforward{(\proj_{2}\times\Id)}\bar\gamma_0(x_0,y)
    \\
    +
    &\max_{\bar\gamma_1\in\setPlans{\gamma}{\bar\mu}}
     \int_{\reals^d\times\reals^d}
    -t c(x_1,y)\d\pushforward{(\proj_{3}\times\Id)}\bar\gamma_1(x_1,y)
    -\frac{\alpha}{2}t(1-t)\wassersteinDistance{2}{\mu_0}{\mu_1}^2
    \end{aligned}
    \\
    &= 
    \begin{aligned}[t]
    &\max_{\tilde\gamma_0\in\pushforward{(\proj_{2}\times\Id)}\setPlans{\gamma}{\bar\mu}}
    \int_{\reals^d\times\reals^d}
    -(1-t)c(x_0,y)\d\tilde\gamma_0(x_0,y)
    \\
    +
    &\max_{\tilde\gamma_1\in\pushforward{(\proj_{2}\times\Id)}\setPlans{\gamma}{\bar\mu}}
     \int_{\reals^d\times\reals^d}
    -t c(x_1,y)\d\tilde\gamma_1(x_1,y)
    -\frac{\alpha}{2}t(1-t)\wassersteinDistance{2}{\mu_0}{\mu_1}^2
    \end{aligned}
    \\
    \overset{\eqref{eq:optimal transport discrepancy alpha convexity property set plans}}&{=}
    \begin{aligned}[t]
    &\max_{\bar\gamma\in\setPlans{\pushforward{(\proj_{2})}\gamma}{\bar\mu}}
    \int_{\reals^d\times\reals^d}
    -(1-t)c(x_0,y)\d\tilde\gamma_0(x_0,y)
    \\
    +
    &\max_{\bar\gamma\in\setPlans{\gamma}{\pushforward{(\proj_{3})}\gamma}}
     \int_{\reals^d\times\reals^d}
    -t c(x_1,y)\d\pushforward{(\proj_{3}\times\Id)}\bar\gamma(x_1,y)
    -\frac{\alpha}{2}t(1-t)\wassersteinDistance{2}{\mu_0}{\mu_1}^2
    \end{aligned}
    \\
    \overset{\eqref{eq:optimal transport discrepancy alpha convexity marginals}}&{=}
    \begin{aligned}[t]
    &\max_{\tilde\gamma_0\in\setPlans{\mu_0}{\bar\mu}}
    \int_{\reals^d\times\reals^d}
    -(1-t)c(x_0,y)\d\tilde\gamma_0(x_0,y)
    \\
    +
    &\max_{\tilde\gamma_1\in\setPlans{\mu_1}{\bar\mu}}
     \int_{\reals^d\times\reals^d}
    -t c(x_1,y)\d\tilde\gamma_1(x_1,y)
    -\frac{\alpha}{2}t(1-t)\wassersteinDistance{2}{\mu_0}{\mu_1}^2
    \end{aligned}
    \\
    &=
    \begin{aligned}[t]
    &-(1-t)\min_{\tilde\gamma_0\in\setPlans{\mu_0}{\bar\mu}}
    \int_{\reals^d\times\reals^d}
    c(x_0,y)\d\tilde\gamma_0(x_0,y)
    \\
    &-t \min_{\tilde\gamma_1\in\setPlans{\mu_1}{\bar\mu}}
     \int_{\reals^d\times\reals^d}
    c(x_1,y)\d\tilde\gamma_1(x_1,y)
    -\frac{\alpha}{2}t(1-t)\wassersteinDistance{2}{\mu_0}{\mu_1}^2
    \end{aligned}
    \\
    &=-(1-t)\cost(\mu_0)-t\cost(\mu_1)-\frac{\alpha}{2}t(1-t)\wassersteinDistance{2}{\mu_0}{\mu_1}^2.
\end{align*}
This proves $\alpha$-convexity of $-\cost$.
\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%
% Proof DRO and std, upper bound (inaccurate)
%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
Then,
\begin{equation*}
\begin{aligned}
    \cost(\mu)
    &=
    \expectedValue{\mu}{\innerProduct{w}{x}}
    + \weight\standardDeviation{\mu}{\innerProduct{w}{x}}
    \\
    &= 
    \innerProduct{w}{\expectedValue{\mu}{x}}
    + \weight \sqrt{\transpose{w}\variance{\mu}{x}w}
    \\
    &= 
    \innerProduct{w}{\expectedValue{\mu}{x}}
    +\weight\norm{\variance{\mu}{x}^{1/2}w}
    \\
    \overset{\triangle}&{\leq}
    \begin{aligned}[t]
    &\innerProduct{w}{\expectedValue{\refmu}{x}} + \norm{w}\norm{\expectedValue{\mu}{x}-\expectedValue{\refmu}{x}}
    \\ &+\weight\norm{\variance{\refmu}{x}^{1/2}w}+\weight\norm{w}\norm{\variance{\mu}{x}^{1/2}-\variance{\refmu}{x}^{1/2}}
    \end{aligned}
    \\
    \overset{\square}&{\leq}
    \cost(\refmu) + \norm{w}\left(\norm{\expectedValue{\mu}{x}-\expectedValue{\refmu}{x}}+\weight\norm{\variance{\mu}{x}^{1/2}-\variance{\refmu}{x}^{1/2}}\right)
    \\
    &=
    \cost(\refmu) + \norm{w}\left(\norm{\expectedValue{\mu}{x}-\expectedValue{\refmu}{x}}+\weight\norm{\variance{\mu}{x}^{1/2}-\variance{\refmu}{x}^{1/2}}_\mathrm{Fro}\right)
    \\
    \overset{\heartsuit}&{\leq}
    \cost(\refmu) + \norm{w}\sqrt{1+\weight^2}\sqrt{\norm{\expectedValue{\mu}{x}-\expectedValue{\refmu}{x}}^2+\norm{\variance{\mu}{x}^{1/2}-\variance{\refmu}{x}^{1/2}}_\mathrm{Fro}^2}
    \\
    \overset{\diamondsuit}&{\leq}
    \cost(\refmu) + \norm{w}\sqrt{1+\weight^2}\wassersteinDistance{2}{\mu}{\refmu}
    \\
    &\leq 
    \cost(\refmu) + \radius\norm{w}\sqrt{1+\weight^2},
\end{aligned}
\end{equation*}
where 
\begin{itemize}
    \item in $\triangle$ we use Cauchy-Schwarz inequality~\cite[Theorem 4.2]{Rudin1987}; 
    \item in $\square$ we use that the Frobenius norm $\norm{\cdot}_\mathrm{Fro}$ of a matrix upper bounds its induced norm $\norm{\cdot}$~\cite{petersen2008matrix}; 
    \item in $\heartsuit$ we use that
        $\sqrt{a^2+b^2}\geq \frac{a+c b}{\sqrt{1+c^2}}$ for all non-negative $a,b,c\in\nonnegativeReals$.
    \item in $\diamondsuit$ we use Gelbrich bound~\cite{Gelbrich1990}:
    If $\mu,\nu\in\Pp{2}{\reals^d}$ with mean $m_1,m_2\in\reals^d$ and covariance matrix $\Sigma_1,\Sigma_2\in\reals^d\times\reals^d$, with $\Sigma_1,\Sigma_2$ symmetric and positive semi-definite, then,
    \begin{equation*}
        \wassersteinDistance{2}{\mu}{\nu}
        \geq 
        \sqrt{\Vert m_1-m_2\Vert^2 + \Vert\Sigma_1^{1/2}-\Sigma_2^{1/2}\Vert_\mathrm{Fro}^2},
    \end{equation*}
    where $\Sigma^{1/2}\in\reals^{d\times d}$ is the unique matrix such that $(\Sigma^{1/2})^2=\Sigma$ and $\norm{\cdot}_\mathrm{Fro}$ is the Frobenius norm.
    \qedhere 
\end{itemize}
\end{comment}

==> old/supplement_dro.tex <==
\section{Relation to Existing Results in \gls{acr:dro}}
Consider the cost function
\begin{equation*}
    \cost(w,\mu)=\expectedValue{\mu}{f(w,x)},
\end{equation*}
and suppose that, for fixed $w$, $f$ is twice continuously differentiable in $x$ and has at most quadratic growth\footnote{Again, one can relax this assumption by requiring that the positive part of $f$ has at most quadratic growth; see discussion in \cref{prop:expectation}}. To ease the notation we will simply write $f(x)$, omitting the dependency on $w$.
We define the \emph{growth rate} of $f$~\cite{Gao2016} as
\begin{equation*}
    \kappa\coloneqq\limsup_{\norm{x}\to\infty}\frac{f(x)}{\norm{x}^2}.
\end{equation*}
Without loss of generality, we assume that $\kappa<+\infty$ or, equivalently, that the supremum is finite; see \cite[Theorem 2]{Yue2021}, \cite[Theorem 1 and Proposition 2]{Gao2016}, and~\cite[Remark 3]{Blanchet2019}. 
Note that, if $f$ has at most quadratic growth, then $\kappa<+\infty$.
Then, by duality for \gls{acr:dro} (see \cite[Theorem 1]{Blanchet2019} and \cite[Theorem 1]{Gao2016}), we have
\begin{equation}\label{eq:dro reformulation}
    \sup_{\mu\in\closedWassersteinBall{2}{\radius}{\refmu}}\expectedValue{\mu}{f(x)}
    =
    \min_{\lambda\geq 0}\lambda\radius^2-\int_{\reals^d}\inf_{x'\in\reals^d}\lambda\Vert x-x'\Vert^2-f(x')\d\refmu(x).
\end{equation}
We assume the supremum is attained by some distribution $\mu^\ast$, and that the solution of the unconstrained problem (i.e., without the constraint $\mu\in\closedWassersteinBall{2}{\radius}{\refmu}$) is not feasible. In turn, this assumptions implies that alla maxima lie at the boundary of the Wasserstein ball and that $\lambda^\ast>0$; see~\cite[Remark 2]{Blanchet2019}.
Moreover, we assume that the growth rate $\kappa$ provides a uniform upper bound for the largest eigenvalue of the Hessian of $f$:
\begin{equation*}
    \kappa\geq\sup_{x\in\reals^d}\frac{\maxEigenvalue{\gradient{}^2f(x)}}{2}.
\end{equation*}
By the following lemma, we can in fact replace the inequality with an equality:
\begin{lemma}
Let $f\in\Ctwo{\reals^d}$ have growth rate $\kappa<+\infty$. 
Assume $\kappa\geq\sup_{x\in\reals^d}\frac{\maxEigenvalue{\gradient{}^2f(x)}}{2}$. Then, 
\begin{equation*}
    \kappa=\sup_{x\in\reals^d}\frac{\maxEigenvalue{\gradient{}^2f(x)}}{2}.
\end{equation*}
\end{lemma}
\begin{proof}
It suffices to prove one inequality. By (multivariate) Taylor's remainder formula
\begin{equation*}
    f(x)=f(0)+\innerProduct{\gradient{}f(0)}{x} + R(x)
    \quad
    \text{with}
    \quad 
    R(x)\leq \frac{\sup_{x\in\reals^d}\maxEigenvalue{\gradient{}^2f(x)}}{2}\norm{x}^2.
\end{equation*}
Then, 
\begin{equation*}
\begin{aligned}[b]
    \kappa
    &= \limsup_{\norm{x}\to \infty}\frac{f(x)}{\norm{x}^2}
    \\
    &\leq \limsup_{\norm{x}\to \infty}\frac{f(0)+\innerProduct{\gradient{}f(0)}{x}+\frac{1}{2}\sup_{x\in\reals^d}\maxEigenvalue{\gradient{}^2 f(x)}\norm{x}^2}{\norm{x}^2}
    \\
    &=\frac{1}{2}\sup_{x\in\reals^d}\maxEigenvalue{\gradient{}^2 f(x)}.
\end{aligned}
\end{equation*}
\end{proof}

By \cite[Corollary 1]{Gao2016}, the existence of an optimal $\mu^\ast$ implies that $\lambda^\ast\geq\kappa$. Under the additional assumption that $\lambda^\ast\neq\kappa$, we can show that optimal solutions of \eqref{eq:dro reformulation} satisfy necessary conditions for optimality:

\begin{proposition}\label{prop:relation classical dro}
Let $\refmu\in\Ppabs{2}{\reals^d}$ be absolutely continuous, assume the supremum in \eqref{eq:dro reformulation} is finite and attained, and 
\begin{equation*}
    \kappa=\sup_{x\in\reals^d}\frac{\maxEigenvalue{{\gradient{}^2f(x)}}}{2}.
\end{equation*}
Let $\lambda^\ast>\kappa$ be a strictly positive optimal solution and consider the well-defined diffeomorphism
\begin{equation*}
    T(x)=\left(\Id-\frac{1}{2\lambda^\ast}\gradient{}f\right)^{-1}(x).
\end{equation*}
Then, $\mu^\ast\coloneqq\pushforward{T}\refmu\in\Pp{2}{\reals^d}$ attains the supremum in \eqref{eq:dro reformulation} and solves the optimality conditions of \cref{thm:wasserstein lagrange multipliers} with $\lambda=\lambda^\ast$.
\end{proposition}

The proof relies on the following technical lemma: 

\begin{lemma}\label{lemma:diffeo}
Let $\varphi\in\Ctwo{\reals^d}$ be strongly convex and $T\coloneqq\gradient{}\varphi$. Then, $T$ is $\Cone{}$-diffeormorphism. Moreover, $T^{-1}$ is the gradient of a strongly convex function.
\end{lemma}

\begin{proof}\
\begin{enumerate}
    \item $T$ is a diffeomorphism:
    By the Hadamard-Caccioppoli theorem~\cite{Gordon1972}, we can show that $T$ is (topologically) proper and that its Jacobian is invertible for all $x\in\reals^d$. Invertibility of the Jacobian of $T$ follows directly from $\varphi$ being strongly convex: since $\gradient{}^2T(x)-\alpha\eye{}$ is positive semidefinite for some $\alpha>0$, all eigenvalues of $\gradient{}^2T(x)$ are larger than $\alpha$, and thus never zero (which implies invertibility). 
    Thus, it suffices to prove that $T$ is proper; i.e., that the preimage of compact set is compact or, equivalently, that $\norm{T(x)}\to+\infty$ as $\norm{x}\to+\infty$. It is well-known that gradients of strongly convex functions are strongly monotone, such that
    \begin{equation*}
        \innerProduct{T(x)-T(0)}{x-0}\geq\alpha\norm{x-0}^2
    \end{equation*}
    for some $\alpha>0$. 
    By Cauchy-Schwartz, $\innerProduct{T(x)-T(0)}{x-0}\leq \norm{T(x)-T(0)}\norm{x}$ and thus
    \begin{equation*}
        \norm{T(x)-T(0)}\geq\alpha\norm{x}.
    \end{equation*}
    Finally, by triangle inequality, $\norm{T(x)}\geq\norm{T(x)-T(0)}-\norm{T(0)}$, which implies
    \begin{equation*}
        \norm{T(x)}\geq\alpha\norm{x}-\norm{T(0)}.
    \end{equation*}
    Clearly, $\norm{T(x)}\to\infty$ as $\norm{x}\to\infty$, which concludes the proof. 

    \item $T^{-1}$ is the gradient of a strongly convex function: it suffices to prove $\gradient{}T^{-1}$ symmetric and that $\gradient{}T^{-1}-\beta\eye{}$ is positive semidefinite for some $\beta>0$. By the inverse function theorem
    \begin{equation*}
        \gradient{}T^{-1}(x)=\left(\gradient{}T(T^{-1}(x))\right)^{-1},
    \end{equation*}
    which is symmetric since $\gradient{}T=\gradient{}^2\varphi$ is symmetric and the inverse of symmetric matrices is symmetric. Moreover, for all $x\in\reals^d$
    \begin{equation*}
        \minEigenvalue{\gradient{}T^{-1}(x)}
        =
        \frac{1}{\maxEigenvalue{\gradient{}T(T^{-1}(x))}}\geq\frac{1}{\alpha}>0.
    \end{equation*}
    Thus, $\gradient{}T^{-1}-\frac{1}{\alpha}\eye{}$ is positive semidefinite, and, since $\frac{1}{\alpha}>0$, we conclude.
\end{enumerate}
\end{proof}

\begin{proof}[Proof of \cref{prop:relation classical dro}]
We proceed in five steps: 
\begin{enumerate}
    \item 
    $T$ is a well-defined $\Cone{}$-diffeomorphism: As the inverse of a diffeomorphism is a diffeomorphism, it suffices to prove that $\Id-\frac{1}{2\lambda^\ast}\gradient{}f$ is a $\Cone{}$-diffeomorphism. By \cref{lemma:diffeo}, it is enough to show that $\Id-\frac{1}{2\lambda^\ast}\gradient{}f$ is the gradient of a strongly convex function or equivalently that all eigenvalues of its Jacobian are larger by some $\alpha>0$ for all $x\in\reals^d$. Note that  
    \begin{equation*}
        \gradient{}\left(\Id-\frac{1}{2\lambda^\ast}\gradient{}f\right)(x)
        =
        \eye{}-\frac{1}{2\lambda^\ast}\gradient{}^2f(x).
    \end{equation*}
    Clearly,
    \begin{equation*}
        \spec\left(\eye{}-\frac{1}{2\lambda^\ast}\gradient{}^2f(x)\right)
        =
        1-\frac{1}{2\lambda^\ast}\spec(\gradient{}^2f(x)).
    \end{equation*}
    Since $\maxEigenvalue{\gradient{}^2f(x)}\leq2\kappa$ uniformly and $\gradient{}^2f(x)$ is symmetric for all $x\in\reals^d$, we have
    \begin{equation*}
        \frac{1}{2\lambda^\ast}\spec(\gradient{}^2f(x))
        \subseteq\frac{1}{2\lambda^\ast}(-\infty,2\kappa]
        =\left(-\infty,\frac{\kappa}{\lambda^\ast}\right]
        \subsetneq(-\infty,1)
        \quad\forall x\in\reals^d,
    \end{equation*}
    and so $\minEigenvalue{\eye{}-\frac{1}{2\lambda^\ast}\gradient{}^2f(x)}\geq 1-\kappa/\lambda^\ast>0$ uniformly. So, $\alpha=1-\kappa/\lambda^\ast>0$.
    
    \item
    $T$ is the optimal transport map from $\refmu$ to $\mu^\ast$: By \cref{lemma:diffeo}, $T^{-1}$ is the gradient of a (strongly) convex function, thus, by \cref{prop:brenier2}, it is the optimal transport map from $\refmu$ and $\mu^\ast$. 
    
    \item 
    $\mu^\ast$ satisfies the optimality conditions with $\lambda^\ast$: recall the the gradient of the objective function is $\gradient{}f$ and that the gradient of the Wasserstein distance is $2(\Id-\optMap{\mu^\ast}{\refmu})=2(\Id-T^{-1})$. It is readily verified that 
    \begin{equation*}
        \gradient{}f=2\lambda\left(\Id - T^{-1}\right).
    \end{equation*}

    \item
    $\mu^\ast$ lies on the boundary of the Wasserstein ball: we need to show that $\wassersteinDistance{2}{\mu^\ast}{\refmu}=\varepsilon$. To start, note that the function $x'\mapsto\lambda\norm{x-x'}^2-f(x')$ is strongly convex in $x$ (for all $x$ and $\lambda$) and thus the function $\lambda\mapsto \min_{x'\in\reals^d}\lambda\norm{x-x'}^2-f(x)$ is continuously differentiable around $\lambda^\ast$ for all $x\in\reals^d$; see~\cite[Theorems 4.13 and 4.14]{Bonnans2000}. So, by Leibniz integration rule, the function
    \begin{equation*}
        \lambda\mapsto \int_{x\in\reals^d}\min_{x'\in\reals^d}\lambda\norm{x-x'}^2-f(x)\d\mu(x)
    \end{equation*}
    is differentiable around $\lambda^\ast$. Indeed, $(\Id-\frac{1}{2\lambda}\gradient{}f)^{-1}$ remains a well defined diffeomorphism for $\lambda$ sufficiently close to $\lambda^\ast$. In particular, it is, by continuity, pointwise dominated by an integrable function and its derivative exists. 
    So, a necessary condition for optimality of the dual reads
    \begin{equation*}
    \begin{aligned}
        \varepsilon^2
        &=
        \diff{}{\lambda}\int_{\reals^d}\lambda\norm{x-\left(\Id-\frac{1}{2\lambda} \gradient{} f\right)^{-1}(x)}^2-f\left(\left(\Id-\frac{1}{2\lambda} \gradient{} f\right)^{-1}(x)\right)\d\refmu(x)
        \\
    \end{aligned}
    \end{equation*}
    Reuse Leibniz integration rule to exchange derivative and integration we obtain
    \begin{equation*}
    \begin{aligned}
        \varepsilon^2
        &=
        \int_{\reals^d}\diff{}{\lambda}\lambda\norm{x-\left(\Id-\frac{1}{2\lambda} \gradient{} f\right)^{-1}(x)}^2-f\left(\left(\Id-\frac{1}{2\lambda} \gradient{} f\right)^{-1}(x)\right)\d\refmu(x)
        \\
        &=
        \begin{aligned}[t]
        &\int_{\reals^d}\norm{x-\left(\Id-\frac{1}{2\lambda}\gradient{} f\right)^{-1}(x)}^2\d\refmu(x)
        \\
        &+2\lambda\int_{\reals^d}
        \left(\left(\Id-\frac{1}{2\lambda} \gradient{} f\right)^{-1}(x)-x\right)\left(\diff{}{\lambda}\left(\Id-\frac{1}{2\lambda} \gradient{} f\right)^{-1}(x)\right)\d\refmu(x)
        \\
        &-2\lambda\int_{\reals^d}\frac{1}{2\lambda}\gradient{}f\left(\left(\Id-\frac{1}{2\lambda} \gradient{} f\right)^{-1}(x)\right)\left(\diff{}{\lambda}\left(\Id-\frac{1}{2\lambda} \gradient{} f\right)^{-1}(x)\right)\d\refmu(x)
        \end{aligned}
        \\
        &=
        \int_{\reals^d}\norm{x-\left(\Id-\frac{1}{2\lambda}\gradient{} f\right)^{-1}(x)}^2\d\refmu(x)
        \\
        &=
        \wassersteinDistance{2}{\mu^\ast}{\refmu}^2,
    \end{aligned}
    \end{equation*}    
    where we used $(\Id-\frac{1}{2\lambda}\gradient{}f)((\Id-\frac{1}{2\lambda}\gradient{} f)^{-1}(x))=x$. Note that this directly implies that $\mu^\ast\in\Pp{2}{\reals}$ by triangle inequality. 

    \item 
    $\mu^\ast$ is optimal: it suffices to check that the cost resulting from $\mu^\ast$ coincides the with optimal value of the dual problem. First, basic rules of integration give
    \begin{equation*}
    \begin{aligned}
        \expectedValue{\mu^\ast}{f(x)}
        &=
        \int_{\reals^d}f(x)\d\left(\pushforward{T}\refmu\right)(x)
        \\
        &=
        \int_{\reals^d}f(T(x))\d\refmu(x).
        \\
        &=
        \lambda^\ast\int_{x\in\reals^d}\norm{x-T(x)}^2\d\refmu(x)
        +
        \int_{x\in\reals^d}
        -\lambda^\ast\norm{x-T(x)}^2+f(T(x))\d\refmu(x).
    \end{aligned}
    \end{equation*}
    By definition of $T$ for fixed $x\in\reals^d$, we have
    \begin{equation*}
        \max_{x'\in\reals^d}-\lambda^\ast\norm{x-x'}^2+f(x')
        =
        -\lambda^\ast\norm{x-T(x)}^2+f\left(T(x)\right),
    \end{equation*}
    where we used that the maximum is attained at $x'=T(x)$.
    Thus, 
    \begin{equation*}
    \begin{aligned}[b]
        \expectedValue{\mu^\ast}{f(x)}
        &=
        \lambda^\ast\int_{x'\in\reals^d}\norm{x-T(x)}^2\d\refmu(x)
        +
        \int_{x\in\reals^d}
        \max_{x\in\reals^d}-\lambda^\ast\norm{x-x'}^2+f(x')\d\refmu(x)
        \\
        &=
        \lambda^\ast\wassersteinDistance{2}{\mu^\ast}{\refmu}^2-\int_{\reals^d}\min_{x'\in\reals^d}\lambda^\ast\norm{x-x'}^2-f(x')\d\refmu(x)
        \\
        &=
        \lambda^\ast\varepsilon^2-\int_{\reals^d}\min_{x'\in\reals^d}\lambda^\ast\norm{x-x'}^2-f(x')\d\refmu(x).
    \end{aligned}
    \end{equation*}
\end{enumerate}
\end{proof}

The proof directly reveals the following corollary:

\begin{corollary}\label{cor:relation classical dro}
Let the assumptions of \cref{prop:relation classical dro} hold. Then, there exists a $\mu^\ast$ attaining the supremum which is absolutely continuous. 
\end{corollary}

\begin{proof}
Since $T$ is a diffeomorphism (in particular, it is injective and the Jacobian has non-zero determinant) and $\refmu$ is absolutely continuous, $\mu^\ast$ is absolutely continuous~\cite[Lemma 5.5.3]{Ambrosio2008a}.
\end{proof}

\begin{remark}\
\begin{enumerate}
    \item
    Many relevant functions satisfy the assumption $\kappa\geq\sup_{x\in\reals^d}\frac{\maxEigenvalue{\gradient{}^2f}}{2}$:
    \begin{enumerate}
        \item linear functions: $\kappa=0$ and $\gradient{}^2f(x)$ is the zero matrix;
        
        \item convex functions whose growth at infinity upper bounds their Hessian (e.g., quadratic functions, but not convex functions such as $x^2+e^{-x^2}$);
        
        \item concave functions: see \cref{prop:relation classical dro concave} for details;
        
        \item functions with norm of the Hessian uniformly bounded via $\frac{1}{2}\sup_{x\in\reals^d}\norm{\gradient{}^2f}\leq\kappa$. 
    \end{enumerate}
    
    \item 
    By \cite[Corollary 1]{Gao2016} an optimal solutions exists only if $\lambda^\ast=0$ or $\lambda^\ast\geq\kappa$. Instead, \cref{prop:relation classical dro} assumes $\lambda^\ast>\kappa$. The case $\lambda^\ast=0$ can be ruled out assuming that the maximum of the unconstrained problem does not lie in the Wasserstein ball; the case $\lambda^\ast=\kappa$ is degenerate and needs to be examined individually.   
    
    \item
    One can replace the assumption $\kappa=\sup_{x\in\reals^d}\frac{\maxEigenvalue{\gradient{}^2f}}{2}$ with the assumption that there exists optimal $\lambda^\ast$ such that $\lambda^\ast>\sup_{x\in\reals^d}\frac{\maxEigenvalue{\gradient{}^2f}}{2}$. Yet, there might not exist a $\lambda^\ast>0$ satisfying the equation.
\end{enumerate}
\end{remark}

The proof can be further strengthened (including $\lambda^\ast=\kappa$) if we additionally assume that $f$ is concave in $x$: 

\begin{proposition}\label{prop:relation classical dro concave}
Let $f\in\Ctwo{\reals}$ and $\refmu\in\Ppabs{2}{\reals^d}$. Assume $f$ is concave. Let $\lambda^\ast\geq\kappa$ be a strictly positive optimal solution and consider the well-defined diffeomorphism
\begin{equation*}
    T(x)=\left(\Id-\frac{1}{2\lambda^\ast}\gradient{}f\right)^{-1}(x).
\end{equation*}
Then, $\mu^\ast\coloneqq\pushforward{T}\refmu\in\Pp{2}{\reals^d}$ attains the supremum in \eqref{eq:dro reformulation} and solves the optimality conditions of \cref{thm:wasserstein lagrange multipliers} with $\lambda=\lambda^\ast$.
\end{proposition}

\begin{proof}
It suffices to show that $\Id-\frac{1}{2\lambda^\ast}\gradient{}f$ is the gradient of a strongly convex function. Then, the proof is identical to the proof of \cref{prop:relation classical dro}. For this, simply observe that, by concavity, all eigenvalue of $\gradient{}^2f(x)$ are non-negative, and thus
\begin{equation*}
    \spec\left(I-\frac{1}{2\lambda^\ast}\gradient{}^2f(x)\right)
    =
    1-\frac{1}{2\lambda^\ast}\spec(\gradient{}^2f(x))
\end{equation*}
and thus $\minEigenvalue{\eye{}-\frac{1}{2\lambda^\ast}\gradient{}f(x)}\geq 1$ for all $x\in\reals^d$. Thus, $\Id-\frac{1}{2\lambda^\ast}\gradient{}f$ is strongly convex.
\end{proof}

Again, proof directly reveals the following corollary, whose proof is identical to the proof \cref{cor:relation classical dro}:

\begin{corollary}\label{cor:relation classical dro concave}
Let the assumptions of \cref{prop:relation classical dro concave} hold. Then, there exists a $\mu^\ast$ attaining the supremum which is absolutely continuous. 
\end{corollary}

\begin{remark}
This result mirrors point (iii) in \cite[Theorem 1]{Gao2016}, stating that, when $f$ is convex, one can restrict the attention to optimal transport maps.
\end{remark}

\begin{comment}
\subsection{Moment-based Ambiguity Sets}
\nlmargin{Consider}{needs to be improved and made meaningful} now the moment-constrained optimization problem
\begin{equation}\label{eq:dro moments}
    \min_{w\in\mathcal{W}}\sup_{\mu\in\mathcal{D}}\expectedValue{\mu}{\innerProduct{w}{x}}+\weight\variance{\mu}{\innerProduct{w}{x}}
\end{equation}
where is
\begin{equation*}
    \mathcal{D}
    \coloneqq 
    \left\{\mu\in\Pp{2}{\reals^d}:\expectedValue{\mu}{\frac{1}{2}\norm{Ax-b}^2}=0\right\}.
\end{equation*}
\end{comment}



\subsection{Solving the \gls{acr:dro} Problem}
So far, we reviewed methods to solve the inner optimization problem~\eqref{eq:general dro}. In this section, we show how this result can be deployed to solve \eqref{eq:general dro} and compute the optimal $w^\ast$. We make the following standard assumption:
\begin{assumption}\label{assumption:regularity full dro}
$\cost(\cdot,\mu)$ is convex and continuously differentiable for all $\mu$ and $w\mapsto\gradient{w}\cost(w,\mu)$ is Lipschitz continuous and bounded by $L$ (uniformly in $\mu$). Finally, $\mathcal{W}$ is convex compact.
\end{assumption}
\cref{assumption:regularity full dro} immediately implies existence of a solution of \cref{eq:general dro}.
For simplicity, let us define
\begin{equation}
\begin{aligned}
    \phi(w)&\coloneqq\max_{\mu\in\closedWassersteinBall{2}{\radius}{\refmu}}\cost(w,\mu) \\
    \mu^\ast(w)&\in\arg\max_{\mu\in\closedWassersteinBall{2}{\radius}{\refmu}}\cost(w,\mu).
\end{aligned}
\end{equation} 
Evaluations of $\phi$ are easy and rely on the theory presented before. 
The next lemma is immediate. 
\begin{lemma}
The function $w\mapsto\phi(w)$ is convex.
\end{lemma}
\begin{proof}
The lemma follows directly from the well-known fact that the supremum of convex functions is convex. 
\end{proof}
While convex, $\phi(w)$ is generally non-differentiable, regardless of the smoothness of $\cost$. Fortunately, we can still prove convergence:
\newcommand{\wopt}{w^\ast}
\newcommand{\wset}{\mathcal{W}}
\newcommand{\witer}[1]{w_{#1}}
\newcommand{\muiter}[1]{\mu^\ast(\witer{#1})}
\newcommand{\stepsizeiter}[1]{\eta_{#1}}
\begin{theorem}[Convergence]
Let $(\stepsizeiter{k})_{k\in\naturals}$ be a sequence of strictly positive real step sizes. Assume
\begin{equation*}
\stepsizeiter{k}\to 0 \text{ and }\sum_{k=0}^\infty\stepsizeiter{k}=\infty.
\end{equation*}
Consider the sequence $(\witer{k})_{k\in\mathbb{N}}$ generated by
\begin{equation}\label{eq:algorithm}
    \witer{k+1}=\projection{\wset}{\witer{k}-\stepsizeiter{k}\gradient{w}\cost(\witer{k},\muiter{k})}
\end{equation}
with $\witer{0}\in\wset$. Then,
\begin{equation*}
    \min_{i=0,\ldots,k}\phi(\witer{i})\to\phi(\wopt) \text{ as } k\to\infty.
\end{equation*}
\end{theorem}
\begin{proof}
The proof follows along the lines of proofs of convergence of subgradient methods.
\begin{comment}
\begin{equation*}
\begin{aligned}
    \phi(\witer{k+1})
    &=
    \max_{\mu\in\closedWassersteinBall{2}{\radius}{\refmu}}J(\witer{k+1},\mu)
    \\
    &\geq
    \cost(\witer{k+1},\muiter{k}) 
    \\
    &\geq 
    \cost(\witer{k},\muiter{k}) + \innerProduct{\gradient{w}J(\witer{k},\muiter{k})}{\witer{k+1}-\witer{k}}
    \\
    &
    =
    \phi(\witer{k}) - \stepsizeiter{k}\norm{\gradient{w}\cost(\witer{k},\muiter{k}}^2,
\end{aligned} 
\end{equation*}
\end{comment}
To start, we use convexity and differentiability of $\cost(\cdot,\mu)$:
\begin{equation}\label{eq:proof algorithm 1}
\begin{aligned}
    \phi(\wopt)
    &=
    \max_{\mu\in\closedWassersteinBall{2}{\radius}{\refmu}}J(\wopt,\mu)
    \\
    &\geq
    \cost(\wopt,\muiter{k}) 
    \\
    &\geq 
    \cost(\witer{k},\muiter{k}) + \innerProduct{\gradient{w}J(\witer{k},\muiter{k})}{\wopt-\witer{k}}
    \\
    &= 
    \phi(\witer{k}) + \innerProduct{\gradient{w}J(\witer{k},\muiter{k})}{\wopt-\witer{k}}.
\end{aligned} 
\end{equation}
Moreover, by non-expansiveness of the projection operator, we get
\begin{equation*}
\begin{aligned}
    \norm{\witer{k+1}-\wopt}^2
    &=
    \norm{\projection{\wset}{\witer{k}-\stepsizeiter{k}\gradient{w}\cost(\witer{k},\muiter{k})}-\projection{\wset}{\wopt}}^2
    \\
    &\leq 
    \norm{\witer{k}-\stepsizeiter{k}\gradient{w}\cost(\witer{k},\muiter{k})-\wopt}^2
    \\
    &=
    \norm{\witer{k}-w^\ast}^2 - 2\stepsizeiter{k}\innerProduct{\gradient{w}\cost(\witer{k},\muiter{k})}{\witer{k}-\wopt}+\stepsizeiter{k}^2\norm{\gradient{w}\cost(\witer{k},\muiter{k})}^2
    \\
    &\leq 
    \norm{\witer{k}-w^\ast}^2 + 2\stepsizeiter{k}(\phi(\wopt)-\phi(\witer{k}))+\stepsizeiter{k}^2\norm{\gradient{w}\cost(\witer{k},\muiter{k})}^2,
\end{aligned}
\end{equation*}
where the last inequality follows from \eqref{eq:proof algorithm 1}.
An inductive argument then leads to 
\begin{equation*}
\begin{aligned}
    \norm{\witer{k+1}-\wopt}^2
    &\leq
    \norm{\witer{1}-\wopt}^2+2\sum_{i=0}^{k}\stepsizeiter{i}\left(\phi(\wopt)-\phi(\witer{i})\right)+\sum_{i=0}^k\stepsizeiter{i}^2\norm{\gradient{w}\cost(\witer{i},\muiter{i})}^2,
\end{aligned}
\end{equation*}
and so to
\begin{equation*}
\begin{aligned}
    2\sum_{i=1}^{k}\stepsizeiter{i}\left(\phi(\witer{i})-\phi(\wopt)\right)
    &\leq
    \norm{\witer{1}-\wopt}^2-\norm{\witer{k+1}-\wopt}^2+\sum_{i=0}^{k}\stepsizeiter{i}^2\norm{\gradient{w}\cost(\witer{i},\muiter{i})}^2
    \\
    &\leq
    \norm{\witer{1}-\wopt}^2+L^2\sum_{i=1}^{k}\stepsizeiter{i}^2.
\end{aligned}
\end{equation*}
As trivially $\min_{i=0,\ldots,k}\phi(\witer{i})-\phi(\wopt)\leq \phi(\witer{i})-\phi(\wopt)$ for all $i$ we therefore conclude
\begin{equation*}
\begin{aligned}
    \min_{i=0,\ldots,k}\phi(\witer{i})-\phi(\wopt)
    \leq 
    \frac{\norm{\witer{1}-\wopt}^2+L^2\sum_{i=0}^{k}\stepsizeiter{i}^2}{2\sum_{i=0}^k\stepsizeiter{i}}.
\end{aligned}
\end{equation*}
The result follows via the assumptions on the step size.
\end{proof}

\begin{remark}\
\begin{enumerate}
    \item In the cases of the mean and mean-variance functionals, it is easy to find (uniform) upper bounds for the gradient.
    
    \item Iteration \eqref{eq:algorithm} resembles a saddle flow with infinitely fast gain for the probability distribution $\mu_k$ (cf. dual ascent methods).
\end{enumerate}
\end{remark}

